A Systematic Investigation of Document Chunking Strategies and Embedding Sensitivity

We present the first large-scale, cross-domain evaluation of document chunking strategies for dense retrieval, addressing a critical but underexplored aspect of retrieval-augmented systems. In our study, 36 segmentation methods spanning fixed-size, semantic, structure-aware, hierarchical, adaptive, and LLM-assisted approaches are benchmarked across six diverse knowledge domains using five different embedding models. Retrieval performance is assessed using graded relevance scores from a state-of-the-art LLM evaluator, with Normalised DCG@5 as the primary metric (complemented by Hit@5 and MRR). Our experiments show that content-aware chunking significantly improves retrieval effectiveness over naive fixed-length splitting. The top-performing strategy, Paragraph Group Chunking, achieved the highest overall accuracy (mean nDCG@5~0.459) and substantially better top-rank hit rates (Precision@1~24%, Hit@5~59%). In contrast, simple fixed-size character chunking as baselines performed poorly (nDCG@5 < 0.244, Precision@1~2-3%). We observe pronounced domain-specific differences: dynamic token sizing is strongest in biology, physics and health, while paragraph grouping is strongest in legal and maths. Larger embedding models yield higher absolute scores but remain sensitive to suboptimal segmentation, indicating that better chunking and large embeddings provide complementary benefits. In addition to accuracy gains, we quantify the efficiency trade-offs of advanced chunking. Producing more, smaller chunks can increase index size and latency. Consequently, we identify methods (like dynamic chunking) that approach an optimal balance of effectiveness and efficiency. These findings establish chunking as a vital lever for improving retrieval performance and reliability.

==> table_0.tex <==
\begin{table*}[t]
\centering
\caption{Embedding models used in this study, with embedding dimensionality.}
\label{tab:emb_models}
\begin{tabular}{l l l r}
\hline
\textbf{Model } & \textbf{Identifier} & \textbf{Dim.} \\
\hline
BGE-M3      & \texttt{BAAI/bge-m3}                    & 1024 \\
MiniLM      & \texttt{all-MiniLM-L6-v2}                  & 384  \\
POTION-8M   & \texttt{minishlab/potion-8M}              & 256  \\
POTION-4M   & \texttt{minishlab/potion-4M}    & 128  \\
POTION-2M   & \texttt{minishlab/potion-2M}                  & 64   \\
\hline
\end{tabular}
\end{table*}

